Stable Distribution Alignment Using the Dual of the Adversarial Distance

Methods that align distributions by minimizing an adversarial distance between them have recently achieved impressive results. However, these approaches are difficult to optimize with gradient descent and they often do not converge well without careful hyperparameter tuning and proper initialization. We investigate whether turning the adversarial min-max problem into an optimization problem by replacing the maximization part with its dual improves the quality of the resulting alignment and explore its connections to Maximum Mean Discrepancy. Our empirical results suggest that using the dual formulation for the restricted family of linear discriminators results in a more stable convergence to a desirable solution when compared with the performance of a primal min-max GAN-like objective and an MMD objective under the same restrictions. We test our hypothesis on the problem of aligning two synthetic point clouds on a plane and on a real-image domain adaptation problem on digits. In both cases, the dual formulation yields an iterative procedure that gives more stable and monotonic improvement over time.

==> experiments_old.tex <==
We also evaluated the performance of proposed model on a visual domain adaptation task. We attempted to adapt a two-layer multi-layered perceptron (MLP) with two hundred hidden units trained to classify a subset of digits from MNIST (source domain) into "fours" and "nines" to perform well in the same task on USPS dataset (target domain).  All images are scaled to 16x16 pixel. 

\begin{figure}[b]
\def \samplefigureimsize {0.20}
\centering
        \includegraphics[width=\samplefigureimsize\textwidth]{figs/real/samples/mnist/4.png}
        \includegraphics[width=\samplefigureimsize\textwidth]{figs/real/samples/mnist/4_1.png}
        \includegraphics[width=\samplefigureimsize\textwidth]{figs/real/samples/mnist/9.png}
        \includegraphics[width=\samplefigureimsize\textwidth]{figs/real/samples/mnist/9_1.png}
\\
        \includegraphics[width=\samplefigureimsize\textwidth]{figs/real/samples/usps/4.png}
        \includegraphics[width=\samplefigureimsize\textwidth]{figs/real/samples/usps/4_1.png}
        \includegraphics[width=\samplefigureimsize\textwidth]{figs/real/samples/usps/9.png}
        \includegraphics[width=\samplefigureimsize\textwidth]{figs/real/samples/usps/9_1.png}
\caption{ Samples from MNIST (first row) and USPS (second row) showing diversity and the domain shift between datasets. Training and testing a two-layer fully-connected network on images from the same domain yields an accuracy above 0.95, but the accuracy drops to 0.5-0.6 when the network is tested on samples from the other domain. This is known as the domain shift problem. }
\label{fig:domain_shift}
\end{figure}

Let us take a closer look at a two-layered MLP domain adaptation architecture we are using below. We will denote the first layer of the MLP as the embedding part and the latter one as the classification part. 

We train different embedding parts - one for each domain, and use a shared classification part. Our architecture also includes a linear discriminator (adversary) that is trained to distinguish features computed by the corresponding embedding parts for different domains.

%BK: This sentence below is confusing to me, and I'm not exactly sure what it means.
After training the source embedding and shared classification part of the network on the source domain, we initialized the target embedding with source embedding weights and optimized the target embedding weights to make the distributions of source and target feature representations less distinguishable. This approach to domain adaptation can be treated as the most basic version of the ADDA architecture \cite{tzeng_cvpr17}. After learning and fixing the source embedding map, we observed that both the negative likelihood objective and the quality of the resulting classifier on the target gradually improved when we were updating target embeddings with the procedure given by the dual linear classifier, but changed quite unexpectedly for a primal linear classifier. Detailed results are shown in \figref{fig:real_results}.

\begin{figure}[t]
\centering
        \includegraphics[width=0.3\textwidth]{figs/real/primal/obj.png}
        \includegraphics[width=0.3\textwidth]{figs/real/primal/daq.png}
        \includegraphics[width=0.3\textwidth]{figs/real/primal/acc.png}
% \\      
        % \includegraphics[width=0.3\textwidth]{figs/real/primal-2/obj.png}
        % \includegraphics[width=0.3\textwidth]{figs/real/primal-2/daq.png}
        % \includegraphics[width=0.3\textwidth]{figs/real/primal-2/acc.png}
\\
%(a) primal case \\
        \includegraphics[width=0.3\textwidth]{figs/real/dual/obj.png}
        \includegraphics[width=0.3\textwidth]{figs/real/dual/daq.png}
        \includegraphics[width=0.3\textwidth]{figs/real/dual/acc.png}
\caption{ Results for the unsupervised domain adaptation of a binary classifier trained to classify digits into nines and fours from MNIST (source domain) and tested on USPS (target domain). Both the negative likelihood objective (first column) and the accuracy of the resulting classifier on target (second column) are not monotonic in the primal case (top row), but show stable improvement over time for the dual case (bottom row). Note that while the discriminator accuracy changes drastically over time in the dual case, the accuracy on target continually improves. The adaptation method based on the dual formulation steadily reaches and retains an accuracy around 0.76, whereas the primal method reached similar accuracy at some point, but also diverged from it over time. These plots were obtained using a basic learning rate scheduling heuristic: divide the learning rate by two if it clearly overshoots on the last step. Without it, results are little worse, but the general trends are still the same. }
\label{fig:real_results}
\end{figure}

%BK: paragraph below is unclear to me; not sure how to fix
These results are encouraging because they show that the training procedure of adversarial unsupervised adaptation could be made more stable.
The stability of the unsupervised adaptation methods is very important because in real-world scenarios we do not have an access to the labeled target set to estimate how the performance of the method changes over time and whether it is converging. Therefore, we are not able to find peak performance on target similar to the one presented in the second column of the first row in Fig. 5. On the other hand, our proposed dual methods can be trained until convergence without the risk of stopping at a sub-optimal solution.

%BK: This paragraph is confusing; not sure how to fix.
% We do not report results for a kernelized version of the same experiment, because it turned out that gradients of the resulting discriminator are vanishingly small, presumably because in higher dimensions  even random initialization of the dual kernel classifier gives a domain discrimination accuracy close to 100\%. This is not an issue for MMD with kernels, because the MMD objective is linear in functional margins, whereas the discriminator objective by design should not distinguish well between high and very high values of functional margin, thus making "high separation" and "very high separation" cases almost indistinguishable in terms of loss value, which in turn makes gradient decent hard for these cases.

% To make the adaptation procedure described above work as expected, we normalize gradients at each step and use a basic heuristic to change the learning rate over time: namely, we decrease the gradient step if on the last step the objective value did not improve, and increase the learning rate if the relative improvement on the last step was below 0.5\%. 

% \begin{figure}[h]
%   \centering
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.9\textwidth]{figs/pics/9.png}
%         \\ (a)
%     \end{minipage}\hfill
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.9\textwidth]{figs/pics/10.png}
%         \\ (b) L2 distance between centers of clouds
%     \end{minipage}\hfill
%     \\
%     \begin{minipage}{0.45\textwidth}    
%         \centering
%         \includegraphics[width=0.9\textwidth]{figs/pics/11.png}
%         \\ (c) discriminator accuracy
%     \end{minipage}\hfill
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.9\textwidth]{figs/pics/12.png}
%         \\ (d) negative likelihood 
%     \end{minipage}\hfill
  % \caption{The shift performed by minimizing adversarial logistic pseudo-distance. Plots show (in clockwise order): the distance between means of distributions, $J(M, w)$ and classification error. Note that even though classification error juggles, as expected, both distance and optimization target $J$ change very steadily.}
% \end{figure}
